Impact of Large-Scale Anisotropies on Galaxy Clustering and Cosmological Constraints

We critically assess the impact of significant dipole and large-scale anisotropies on galaxy clustering signals, with a focus on radio continuum surveys. Our study reveals that these anisotropies -- resulting from intrinsic cosmological effects and/or observational systematics -- profoundly influence the two-point correlation function (2PCF) and angular power spectrum ($C_\ell$). Notably, large-scale anisotropies can obscure or simulate non-Gaussianity signals, complicating the extraction of precise cosmological information. The results emphasize that it is crucial to address systematics and rigorously mask the dipole and its surrounding multipoles to obtain accurate cosmological constraints. This approach is essential for extracting cosmological results from clustering signals, particularly for future surveys such as SKA, DESI, and LSST, to ensure the precision and reliability of cosmological analyses.

==> def.tex <==
\usepackage[ngerman,english]{babel}
\newif\ifAMStwofonts
\AMStwofontstrue 
\def\degr{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\vgrad{{\bf \nabla}}
\def\pesc{{\rm P}_{\rm esc}}
\def\fsnr{{\rm f}_{\rm _{SNR}}}
\def\aobs{{\alpha_{\rm _{obs}}}}
\def\baobs{{{\bar\alpha}_{\rm _{obs}}}}
\def\bz{{b(z)}}
\def\nz{{N(z)}}
\def\cl{{C_\ell}}
\def\cln{{C^n_\ell}}
\def\clth{{C^{\rm th}_\ell}}
\def\clobs{{C^{\rm obs}_\ell}}
\def\clcorr{{C^{\rm corrected}_\ell}}
\def\dl{{d_{\ell m}}}
\def\al{{a_{\ell m}}}
\def\almo{{a^{\rm obs}_{\ell m}}}
\def\tal{{{\tilde a}_{\ell m}}}
\def\dl{{d_{\ell m}}}
\def\vPsi{{\bf \Psi}}
\def\vPhi{{\bf \Phi}}
\def\vmu{{\bm \mu}}
\def\wpdot{W_{{\dot \phi}}}
\def\wph{W_{ \phi}}
\def\wv{W_{ \rm V}}
\def\cA{${\cal A}$}
\def\caM{{\cal M}}
\def\rmin{{r_{_{\rm min}}}} 
\def\rmax{{r_{_{\rm max}}}} 
\def\rz{{r}} 
\def\vh{{v_{_{\rm h}}}} 
\def\Vs{{V_{_{\rm seed}}}} 
\def\Vsi{{V_{_{{\rm seed},i }   }}} 
\def\As{{a_{_{\rm seed}}}} 
\def\Asj{{a^j_{_{\rm seed}}}} 
\def\zcos{z_{_{\rm cos}}}
\def\Ps{{P_{_{\rm seed}}}} 
\def\Psii{{P_{_{{\rm seed},i} }}} 
\def\sigint{\sigma_{\eta,{\rm int}}}
%\def\ssigint{\sigma^2_{\eta,{\rm int}}}
\def\ssigint{\sigma^2_{\eta}}
\def\cBo{{\cal B}_{\rm o}}
\def\cBt{{\cal B}_{\rm t}}
\def\Pm{{P_{_{\rm m}}}} 
\def\ti{{t_{_{0}}}} 
\def\Pa{{P_{_{\alpha}}}} 
\def\Qks {{Q_{_{\rm KS}}}} 
\def\rcu{ {r_{_{\rm cut}} }}
\def\md{ {M_{_{\rm disk}} }}
\def\psid{ {\Psi_{_{\rm disk}} }}
\def\psih{ {\Psi_{_{\rm halo}} }}
\def\kpc{ {\; {\rm kpc}}}
\def\Ns{N_{\rm s}}
\def\caH{{\cal H}}
\def\fg{{f_{_{\rm g} }}}
\def\fdm{{f_{_{\rm DM} }}}
\def\fgz{{f_{_{\rm g17} }}}
\def\etaz{{\eta_{_{\rm 01} }}}
\def\caS{{\cal S}}
\def\wp{{w_{+}}}
\def\wm{{w_-}}
\def\mup{{\mu_+}}
\def\sigmatwo{{\sigma_{_{2}}}}
\def\mum{{\mu_-}}
\def\nup{{\nu_+}}
\def\num{{\nu_-}}
\def\lp{{\lambda_+}}
\def\lm{{\lambda_-}}
\def\vnabla{\bm{\nabla}}
\def\vv{\bf v}
\def\vu{\bf u}
\def\vB{{\bf B}}
\def\eeth{ E_{_{\rm th}} } 
\def\mm{M_{\rm m}}
\def\ms{M_{\rm s}}
\def\Vp{{V_+}}
\def\Vm{{V_-}}
\def\gsim{~\rlap{$>$}{\lower 1.0ex\hbox{$\sim$}}}
\def\xm{x_{_{\rm M}}}
\def\tdmj{{\tilde \varrho}_{{\rm M}j}}
\def\td{t_{_{\rm d}}}
\def\tobs{t_{_{\rm obs}}}
\def\simpropto{\lower.2ex\hbox{$\; \buildrel \propto \over \sim \;$}}
\def\ltsim{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\def\gtsim{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\ltsim{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\def\gtsim{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\th{\theta}
\def\tht{\tilde \theta}
\def\cv{ v}
\def\cvt{ \tilde v}
\def\wt{ \tilde w}
\def\ut{ \tilde u}
\def\dotr{\dot {\bf r}}
\def\ni{\noindent}
\def\gm{\gamma}
\def\pa{\partial}
\def\vm{{\langle v_{12}\rangle_{{\rm m}} }} 
\def\vg{v_{_{\rm g}}}
\def\ag{a_{_{\rm g}}}
\def\aitf{a_{_{\rm itf}}}
\def\vmle{\vB_{_{\rm MLE}} }
\def\vace{\vB_{_{\rm ASCE}} }
\def\vF{{\bf F}}
\def\Rv{R_{\rm v}}
\def\vnabla{{\bf \nabla}}
\def\gmp{\gamma_\|}
\def\gmt{\gamma_\perp}
\def\sgt{\sigma_\perp}
\def\sgls{\sigma_{ls}}
\def\bfeta{{\bf \eta}}
\def\stream{{\langle v_{12}(r)\rangle}}   
\def\H{{\cal H}}
\def\He{{\cal H}{\rm e}}
\def\za{{Zel'dovich approximation}}
\def\cm{\,{\rm cm}}
\def\erg{\,{\rm erg}}
\def\Hz{\,{\rm Hz}}
\def\sr{\,{\rm sr}}
\def\s{\,{\rm s}}
\def\K{\,{\rm K}}
\def\sv{\Theta{^{\rm V}}}
\def\sw{\Theta{^{\rm \Phi}}}
\def\sisw{\Theta{^{\rm { \dot \Phi}}}}
\def\tsv{{\tilde \Theta}{^{\rm V}}}
\def\tsw{{\tilde \Theta}{^{\rm \Phi}}}
\def\tsisw{{\tilde \Theta}{^{\rm { \dot \Phi}}}}
\def\sun{\Theta_{_{\rm un}}}
\def\fsk{f_{_{\rm sky}}}
  \def\rg{\rho_{_{\rm g}}}
    \def\rdm{\rho_{_{\rm dm}}}
\def\kms{\mbox{km\,s$^{-1}$}}
\newcommand{\Mpc}{\, {\rm Mpc} }
\def\Msol{\mbox{M$_\odot$}}
%\def\mg{\mbox{M$_{\rm g}$}}
%\def\mbh{\mbox{M$_{\rm bh}$}}
%\def\mp{\mbox{M$_{\rm p}$}}
%\def\mg{ M_{_{\rm g}} }
%\def\mbh{ M_{_{\rm BH}} }
%\def\mbht{ M_{_{\rm BH,8 }} }
\def\mg{ M_{{ g}} }
\def\mbh{ M_{{BH}} }
\def\mbht{ M_{{ BH,8 }} }
%\def\mdm{ M_{_{\rm DM}} }
\def\mdm{ M_{{DM}} }
\def\prd{Physical Review D.}
\def\nat{Nature}
\def\astjo{Astronomical Journal}
\def\mp{ m_{_{\rm p}} }
\def\sigT{ \sigma_{_{\rm T}} }
\def\bigexpec#1{\biggl \langle#1\biggl \rangle}
\def\expec#1{\langle#1\rangle}
\def\dd{\,{\rm d}}
\def\dhik{(n_{{_{\rm HI}}})_{k}}
\def\rb{{R_{_{\rm b}}}}
\def\gammab{\gamma_{_{\rm b}}}
\def\vb{{v_{_{\rm b}}}}
\def\nb{{n_{_{\rm b}}}}
\def\rs{{r_{_{\rm s}}}}
\def\ngal{{n_{_{\rm gal}}}}
\def\bnb{{{\bar n}_{_{\rm b}}}}
\def\pb{{p_{_{\rm b}}}}
\def\pam{{p_{_{\rm a}}}}
\def\eb{{E_{_{\rm b}}}}
\def\ebi{{E_{_{\rm bi}}}}
\def\pbi{{p_{_{\rm bi}}}}
\def\rbi{{R_{_{\rm bi}}}}
\def\rhob{{\rho_{_{\rm b}}}}
\def\rhov{{\rho_{_{\rm v}}}}
\def\gN{g_{_{\rm N}}}
\def\gM{g_{_{\rm M}}}
%\parskip 6pt
%\overfullrule = 0pt
\def\np{\vfill\eject}
\def\no{\noindent}
\def\bk{\hfill\break}
%       The following macros should be used only in math mode.
\def\ergcms{\,{\rm erg\,cm^{-3}\,s^{-1}}}
\def\kms{\ {\rm km\,s^{-1}}}
\def\hmpc{\ {\rm h^{-1}Mpc}}
\def\hh{\ {\rm h_{50}}}
\def\hmmpc{\ {\rm h\,Mpc^{-1}}}
\def\gcc{\,{\rm g\,cm^{-3}}}
\def\tl{ {\tilde l}}
\def\pcc{\,{\rm cm^{-3}}}
\def\kel{\,{\rm K}}
\def\dd{{\rm d}}
\def\nb{{\bar n}}
\def\ln{{\rm ln}}
\def\pa{\partial}
\def\rarrow{\rightarrow}
\def\larrow{\leftarrow}
%\def\la{\langle}
%\def\ra{\rangle}
\def\grad{\nabla}
%
\def\pmb#1{\setbox0=\hbox{#1}%
\kern-.025em\copy0\kern-\wd0
\kern.05em\copy0\kern-\wd0
\kern-.025em\raise.0433em\box0}
\def\th{\vartheta}
%\def\vth{\vec\th}
\def\vth{\pmb{$\th$}}
\def\ph{\varphi}
 \def\disw{\Theta_{_{\rm  ISW}}}

\def\phv{\ph_v}
\def\phg{\ph_g}
\def\vV{\pmb{V}}
\def\vv{\pmb{v}}
\def\vL{\pmb{L}}

\def\vs{\pmb{s}}
\def\vq{\pmb{q}}
\def\vx{\pmb{x}}
\def\vr{\pmb{r}}
\def\vn{\pmb{n}}
\def\hvn{\hat {\vr}}

%\def\vg{\pmb{$g$}}
\def\vk{\pmb{k}}
\def\hvk{\hat {\vk}}
\def\vaj{\pmb{\alpha}}
\def\vpsi{\pmb{\psi}}
\def\phiv{\phi_v}
\def\phig{\phi_g}
\def\pot {\Phi}
\def\iras {{\it IRAS~}}
\def\velmod{VELMOD~}
%\def\Ft {{\         }}
%\def\tj {{\wpdot}}
\def\Ft {{F}}
\def\tj{{F}}

\def\ajj {{a}^j}
\def\aj{AJ}
\def\gh{\gamma_{_{*}}}  \def\ah{\alpha_{_{*}}}  \def\bh{\beta_{_{*}}}
\def\Nh{N_{_{*}}} 
\def\ajp {{\psi}^{j'}}
\def\ip {i^\prime}
\def\jp {j^\prime}
\def\bfr {{\bf r}}
\def\etal{{\it et al.\ }}
\def\con {5\log {\rm e}}
\def\simlt{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\def\simgt{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\Msun{\rm\> M_{\odot}}
%\def\vnabla{\vec\nabla}
\def\vnabla{\pmb{$\nabla$}}
\def\vitf{v_{_{\rm itf} }}
\def\void#1{{#1}}
%\include{rotating}
\newcommand{\beq}{\begin{equation}}

\newcommand{\eeq}{\end{equation}}
\def\beqa{\begin{eqnarray}}
\def\eeqa{\end{eqnarray}}
%\def\la{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
%\def\ga{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\fixit#1{}
\def\hmpc{h^{-1}\,{\rm Mpc}}
\def\hkpc{h^{-1}\,{\rm kpc}}
\def\dd{{\rm d}}
\def\apj{ApJ}
\def\jcap{JCAP}
\def\prl{Physical Review Letters}
\def\astroj{Astrophysical. J}
\def\aapr{A\&A Rev.}
\def\aaps{A\&AS}
\def\apjs{ApJ. S}
\def\cN{{\cal N}}
\def\cn{{\cal n}}
\def\cS{{\cal S}}
\def\physrep{Physics Reports}
\def\apjl{ApJL}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\araa{ARAA}
\def\prd{Physical Review D.}
\def\nat{Nature}
\def\apjl{ApJL}
\def \ssr{Space Science Reviews}
\def \pasa {Publ. Astron. Soc. Aust.}
%\usepackage{lscape}
%\input{definitions}

\def\file#1{\texttt{#1}}
\def\mudm{\mu_{_{\delta\! M_*}}}
\def\sigdm{\sigma_{_{\delta\! M_*}}}
\def\mual{\mu_{_{\delta\! \alpha}}}
\def\sigal{\sigma_{_{\delta\! \alpha}}}

\def\muas{  \mu  as}
\def\muasyr{\mu as \, {\rm yr}^{-1} }


